Generating medically-accurate summaries of patient-provider dialogue: A multi-stage approach using large language models

A medical provider's summary of a patient visit serves several critical purposes, including clinical decision-making, facilitating hand-offs between providers, and as a reference for the patient. An effective summary is required to be coherent and accurately capture all the medically relevant information in the dialogue, despite the complexity of patient-generated language. Even minor inaccuracies in visit summaries (for example, summarizing "patient does not have a fever" when a fever is present) can be detrimental to the outcome of care for the patient. This paper tackles the problem of medical conversation summarization by discretizing the task into several smaller dialogue-understanding tasks that are sequentially built upon. First, we identify medical entities and their affirmations within the conversation to serve as building blocks. We study dynamically constructing few-shot prompts for tasks by conditioning on relevant patient information and use GPT-3 as the backbone for our experiments. We also develop GPT-derived summarization metrics to measure performance against reference summaries quantitatively. Both our human evaluation study and metrics for medical correctness show that summaries generated using this approach are clinically accurate and outperform the baseline approach of summarizing the dialog in a zero-shot, single-prompt setting.

==> sections/abstract_notes.tex <==
%A medical provider's summary of a patient visit serves several critical purposes, including clinical decision making, facilitating hand-offs between providers, and as a reference for the patient. Recent advances in large language models (LLMs) have enabled summarization models that produce general-domain summaries that both show improvements on benchmarks and are frequently preferred by human evaluators \cite{goyal2022news}.  However, this success is difficult to translate to the medical domain, given the presence of highly domain-specific terminology and the need for clinical precision.  

%Therefore we introduce a multi-stage framework that produces a precise clinical encounter summary, building off of GPT-3 (davinci-003). Our framework discretizes the task of summarization into several, smaller dialogue understanding tasks that are sequentially built upon. We also dynamically construct few-shot prompts for tasks by conditioning on relevant patient information.  We show that summaries generated using this framework are clinically accurate, and that the discretization of summarization in this manner outperforms zero-shot \TODO{we say zero-shot because that is what we compared to?} summarization on the dialogue alone.

%Recent advances in large language models (LLMs) have enabled summarization models that produce general-domain summaries that both show improvements on benchmarks and are frequently preferred by human evaluators \cite{goyal2022news}. However, this success is difficult to translate to the medical domain, given the presence of highly domain-specific terminology and the need for clinical precision.  

%We hope that our work demonstrates how progress in LLMs can be impactful in medicine.


%Clinical encounter summarization between a medical provider and a patient is critical to recording details used in clinical decision making and for facilitating handoffs between kinds of providers. Summarization can take several minutes per encounter and accumulate to several hours of charting work per week, of which increased levels have been associated with higher rates of physician burnout. \cite{eschenroeder2021Associations}

%Large language models (LLMs) have shown success on summarization benchmarks, however, such success has been difficult to translate to the medical domain due to the need to handle highly domain-specific terminology and the need for high clinical precision.
 
%In this work, we use GPT-3 (davinci-002) to introduce a multi-stage framework that produces a precise clinical encounter summary. Our framework discretizes the task of summarization into several, smaller dialogue understanding tasks that build on each other’s outputs. We also dynamically construct few-shot prompts for each task by conditioning on relevant patient information.

%We show that summaries generated using this framework are clinically accurate, and that the discretization of summarization in this manner outperforms naive summarization on the dialogue alone. We hope that our work demonstrates how progress in LLMs can directly contribute to reduced physician overhead in providing quality care.

==> sections/related_work.tex <==
\section{Related Work}
Advances in large language model research \cite{brown2020gpt3, lewis-etal-2020-bart} has in turn lead to widespread advances in natural language processing \cite{Agrawal2022LargeLM,dou-etal-2022-gpt,gao-etal-2022-precise}. Improvements also have been shown when applying large language models to summarization for a variety of non-medical domains \cite{goyal2022news,bhskar-etal-2022-opinion,sclar2022referee}, including some that leverage external resources \cite{narayan-etal-2021-planning}.

While generating from a LLM can produce high-quality results with a single, static prompt, later work has shown that proving the model with examples relevant to the specific input during inference \cite{brown2020gpt3}.  This allows for general-task models to be tailed for a specific task without finetuning the model \cite{min-etal-2020-demonstrations}.  In addition, breaking down the task into several prompts, called \textit{chaining}, allows for subtasks to be discretely processed, and for additional interpretability by providing output at each step \cite{wu2022AIChains}.
%\subsubsection{Discretized and Dynamic Prompting}

The task of summarization in clinical text has been studied prior to the advent of large language models \cite{pivovarov-elhadad-2015-automated}.  
Neural methods have led to better quality summaries \cite{liang-etal-2019-novel-system, gao-etal-2022-summarizing}, including approaches that \citet{macavaney2019ontology} highlight the utility of information from a clinical knowledge base. 

The task of clinical dialogue summarization builds upon the challenges present in general clinical summarization, but adds the additional challenge of including patient-generated text.  However, the application of deep learning methods which leverage external resources have found similar success \cite{enarvi-etal-2020-generating}.  These include \citet{joshi-etal-2020-dr}, which uses a pointer generation model combined with explicit negation and knowledge base information.  Relatedly, \cite{zhang2021leveraging} fine-tunes a BART model on doctor-patient dialogues, which leads to a high-performing model.

==> sections/result_tables.tex <==
\begin{table*}[ht!]
    \centering
%     \resizebox{1.0\textwidth}{!}
%     {
%     % Please add the following required packages to your document preamble:
% % \usepackage{multirow}
%     % \begin{tabular}{c c c c c c c c c}
%     % \toprule
%     % \multirow{2}{*}{Method}&\multirow{2}{*}{K-shot}&\multirow{2}{*}{K-shot Method}&\multirow{2}{*}{Unknown Entity Resolver}& \multicolumn{5}{c}{GPT-F1 ($\uparrow$)} \\
%     % & & & & Pertinent Positives & Pertinent Negatives & Pertinent Unknowns & Medical History & Average\\
%     % \hline
%     % \multirow{3}{*}{Naive}& 0-shot & - & - & \textbf{72.9} & \textbf{71.7} & 45.4 & 43.9 & 58.5 \\
%     % & 1-shot & semantic & - & 71.0 & 69.5 & 42.1 & 48.3 & 57.7 \\
%     % & 1-shot & random & - & 69.4 & 69.1 & 47.5 & 44.7 & 57.7 \\
%     % \hline
%     %   &  1-shot & semantic & \checkmark & 72.4 & 70.1 & 50.0 & 46.2 & 59.7\\
%     %   &  3-shot & semantic & \checkmark & 71.9 & 69.0 & 42.5 & 47.0 & 57.6\\
%     %   &  5-shot & semantic & - & 72.8 & 68.3 & 44.2 & 47.5 & 58.2\\
%     %  MEDSUM & 5-shot & semantic & \checkmark & 71.8 & 70.2 & 46.6 & 46.3 & 58.7\\
%     %   &  1-shot & random & \checkmark &  71.4 & 71.1 & 54.0 & 48.3 & 61.2\\
%     %   &  3-shot & random & \checkmark & 72.2  & 70.9 & \textbf{55.8} & \textbf{50.4} & \textbf{62.3}\\
%     %   &  5-shot & random & \checkmark & 71.9 & 68.3 & 51.9 & 48.2 & 60.0\\
%     % \bottomrule
%     % \end{tabular}
%     }
    \resizebox{1\textwidth}{!}
    {
%\begin{tabular}{cccccccccc}
\begin{tabular}{cP{1.5cm}P{2.2cm}P{1.5cm}P{1.5cm}|P{1.5cm}P{1.8cm}P{1.8cm}P{1.5cm}P{1.5cm}}
\toprule
%\multirow{2}{*}{Method} & \multicolumn{3}{c}{K-shot} & \multirow{2}{*}{Entity Resolver} & \multicolumn{5}{c}{GPT-F1 ($\uparrow$)} \\
% & Extraction & Summarization & Method &  & Pertinent Positives & Pertinent Negatives & Pertinent Unknowns & Medical History & Average \\ \hline
 &  & & &  & \multicolumn{5}{c}{GPT-F1 ($\uparrow$)} \\
Method & Extraction K-shot & Summarization K-shot & Example Selection & Entity Resolver & Pertinent Positives & Pertinent Negatives & Pertinent Unknowns & Medical History & Average\\ \hline
\multirow{3}{*}{Naive} & - & 0-shot & - & - & \textbf{72.9} & \textbf{71.7} & 45.4 & 43.9 & 58.5 \\
 & - & 1-shot & semantic & - & 71.0 & 69.5 & 42.1 & 48.3 & 57.7 \\
 & - & 1-shot & random & - & 69.4 & 69.1 & 47.5 & 44.7 & 57.7 \\\hline
\multirow{7}{*}{MEDSUM} & 1-shot & 1-shot & semantic & \checkmark & 72.4 & 70.1 & 50.0 & 46.2 & 59.7 \\
 & 1-shot & 1-shot & random & \checkmark & 71.4 & 71.1 & 54.0 & 48.3 & 61.2 \\
 & 3-shot & 1-shot & semantic & \checkmark & 71.9 & 69.0 & 42.5 & 47.0 & 57.6 \\
 & 3-shot & 1-shot & random & - & 72.1 & 69.4 & 46.4 & 45.8 & 62.3 \\
  & 3-shot & 1-shot & random & \checkmark & 72.2 & 70.9 & \textbf{55.8} & \textbf{50.4} & \textbf{62.3} \\
 & 5-shot & 1-shot & semantic & \checkmark & 71.8 & 70.2 & 46.6 & 46.3 & 58.7 \\
 & 5-shot & 1-shot & random & \checkmark & 71.9 & 68.3 & 51.9 & 48.2 & 60.0 \\ \bottomrule
\end{tabular}
}
    \caption{Results of GPT-driven metrics. Performance across "Pertinent Positives", "Pertinent Negatives" sections are fairly consistent across methods. MEDSUM demonstrates consistently improved performance in the "Pertinent Unknowns" and "Medical History" sections. Surprisingly, we also find consistently higher performance across experiments using random in-context example selection over semantic-similarity based selection.
}
    \label{table:table_1}
\end{table*}
